Quantifying Intrinsic Uncertainty in Classification via Deep Dirichlet Mixture Networks

With the widespread success of deep neural networks in science and technology, it is becoming increasingly important to quantify the uncertainty of the predictions produced by deep learning. In this paper, we introduce a new method that attaches an explicit uncertainty statement to the probabilities of classification using deep neural networks. Precisely, we view that the classification probabilities are sampled from an unknown distribution, and we propose to learn this distribution through the Dirichlet mixture that is flexible enough for approximating any continuous distribution on the simplex. We then construct credible intervals from the learned distribution to assess the uncertainty of the classification probabilities. Our approach is easy to implement, computationally efficient, and can be coupled with any deep neural network architecture. Our method leverages the crucial observation that, in many classification applications such as medical diagnosis, more than one class labels are available for each observational unit. We demonstrate the usefulness of our approach through simulations and a real data example.

==> method.tex <==
\section{Dirichlet Mixture Networks}
In this section, we introduce the Dirichlet mixture networks, highlighting their flexibility of dealing with a large range of uncertainty quantification tasks. We begin with the case of binary classification, where Dirichlet mixtures reduce to the simpler Beta mixtures. Although perhaps the simplest example, the binary case is sufficient to capture all ingredients of our general approach and, thus, no generality is lost. For completeness, extensions to the multi-class case are considered in Section \ref{sec:extens-mult-labels}.

\begin{figure}[h]
\centering
\includegraphics[width=8cm]{images/introduction.PNG}
\caption{Illustration of the setting. Two or more labels are generated with the \textit{same} probability $p_x$, which is \textit{randomly} drawn from a distribution that we wish to estimate.}
\label{fig:cat}
\end{figure}

%%The high-level idea of our work is that having a single label is insufficient for quantifying uncertainty in many tasks. For example, imagine that one coin yields the head with probability 50\%, and the other is a mixture coin: with weight $0.5$, the head is observed with probability 75\%, and with the rest $0.5$ weight, the head is observed with probability 25\%. It is easy to show that a single toss is statistically impossible to distinguish between the two coins, while two or more tosses are sufficient.
%%corresponding to the Beta mixture networks (BMN), captures all ingredients of the Dirichet mixutre networks. Recognizing this, we start by introducing the BMN and then turn to DMN.

%\subsection{Universal Approximation}
%\label{sec:universaility}


%% First, we would like to denote some notation: a beta distribution with parameters $\alpha$ and $\beta$ is denoted as $\mathscr{B}(\alpha, \beta)$; also 
%% and $f_{\omega}$ the density function of Beta mixture distribution:
% \begin{align}
% f_{\omega} = \sum_{k \geq 1} p_k \mathscr{B}(\alpha_k, \beta_k)
% \end{align}

Let $\{1, 2\}$ denote the two classes. Given an observational unit $x$ (e.g., the image in Figure~\ref{fig:cat}), our model assumes that the probability $p_x$ that $x$ belongs to the first class is a \textit{random variable}, instead of a deterministic value in $[0, 1]$. Denote by $f(p; x)$ defined on $[0, 1]$ the probability density function of $p_x$, which encodes the \textit{intrinsic} uncertainty of the classification problem. In particular, merely knowing the mean probability $\int_0^1 f(p) \dx p$ is not sufficient for informed decision-making. For example, it can happen that, for $x, x'$, their mean probabilities are the same but the densities are far apart from each other.  

Our Dirichlet mixture networks aim to estimate the density function $f(p;x)$ for each $x$. We begin by introducing the loss function to be minimized via deep learning as below.

\subsection{Loss function}\label{sec:likelihood}

%%Denote by $p_x$ the probability of the label being 1 given $x$. For the moment, assume that the random variable $p_x$ follows a Beta mixture distribution whose probability density is
%%general case where $p(x)$ might not be generated from a Beta (finite) mixture distribution.
%% Our model is probabilistic in nature and its negative log-likelihood function serves as the loss function used in the mixture networks. 
% \begin{equation}\label{eq:full_like}
% -\ell(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K;  x_1, \bm y_1, \ldots, x_n, \bm y_n) = -\sum_{j=1}^n \log \left[\sum_{k=1}^K \frac{w^k(x_j)\B(\alpha^k_1(x_j)  + S_{1j}, \alpha^k_2(x_j) + S_{2j})}{\B(\alpha^k_1(x_j), \alpha^k_2(x_j))} \right].
% \end{equation}

A difficulty arising from this estimation problem is that $f$ in general can be any density function on $[0, 1]$. Recognizing this difficulty, we propose to simplify the problem by restricting our focus to the case where $f$ is a Beta mixture:
\begin{equation}\label{eq:beta_density_mix}
f(p; x) = \sum_{k=1}^K w^k \frac{p^{\alpha^k_1 -1} (1-p)^{\alpha^k_2 -1}}{\B(\alpha^k_1, \alpha^k_2)},
\end{equation}
where $\B(\cdot, \cdot)$ is the Beta function, and the parameters $w^k, \bm\alpha^k = (\alpha^k_1, \alpha^k_2)$ are (smooth) functions of $x$, that is, $w^k = w^k(x), \alpha^k_1 = \alpha^k_1(x)$, and $\alpha^k_2 = \alpha^k_2(x)$. The weights $w^k$ satisfy $w^1 + \cdots + x^K = 1$. With this density form in place, our goal is to estimate the parameters $\alpha_1^k, \alpha_2^k > 0$, and $w^k$ for $1 \le k \le K$. Before proceeding to the next step, it is worth pointing out that the restriction on the density function class is nearly harmless due to the universal approximation of Beta mixtures. Section~\ref{sec:universaility} will discuss this in detail.

The next step is to obtain the negative log-likelihood function, which serves as the the loss function used in the mixture networks. Let $x_1, \ldots, x_n$ be the features of $n$ observational units, each of which are associated with labels $y_j^{(1)}, \ldots, y_j^{(m_j)}$ taking values from $\{1, 2\}$ for $1 \le j \le n$. Through integrating out $p$, the likelihood of $w^k, \bm\alpha^k$ for the observed pair $x_j, \bm y_j = (y_j^{(1)}, \ldots, y_j^{(m_j)})$ is 
\[
\begin{aligned}
&L_j(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K; x_j, \bm y_j) \\
&= \int_0^1 p^{\sum_{l=1}^{m_j} \bm{1}(y_j^{(l)}= 1)} (1-p)^{\sum_{l=1}^{m_j} \bm{1}(y_j^{(l)}=2)} f(p; x_j)  \dx p.
\end{aligned}
\]
Write $S_{ij} = \sum_{l=1}^{m_j} \bm{1}(y_j^{(l)} = i)$ for $i = 1, 2$ and $j = 1, \ldots, n$. Note that $S_{ij}$ is the number of times $x_j$ is labeled $i$. Plugging \eqref{eq:beta_density_mix} into the latest display gives
\[
\begin{aligned}
&L_j(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K; x_j, \bm y_j)\\
&= \int_0^1 p^{S_{1j}} (1-p)^{S_{2j}} \sum_{k=1}^K \frac{w^k p^{\alpha^k_1 -1} (1-p)^{\alpha^k_2 -1}}{\B(\alpha^k_1, \alpha^k_2)} \dx p\\
   &= \sum_{k=1}^K \int_0^1 \frac{w^k}{\B(\alpha^k_1, \alpha^k_2)}  p^{\alpha^k_1 -1 + S_{1j}} (1-p)^{\alpha^k_2 -1 + S_{2j}} \dx p.
\end{aligned}
\]
Making use of a basic property of Beta functions, we get
\[
L_j(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K; x_j, \bm y_j)  = \sum_{k=1}^K \frac{w^k\B(\alpha^k_1  + S_{1j}, \alpha^k_2 + S_{2j})}{\B(\alpha^k_1, \alpha^k_2)}.
\]
Aggregating all the $n$ observed units, we finally obtain the full negative log-likelihood given as
\begin{equation}\label{eq:full_like}
\begin{aligned}
&-\ell(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K;  x_1, \bm y_1, \ldots, x_n, \bm y_n) = \\
&-\sum_{j=1}^n \log \left[\sum_{k=1}^K \frac{w^k(x_j)\B(\alpha^k_1(x_j)  + S_{1j}, \alpha^k_2(x_j) + S_{2j})}{\B(\alpha^k_1(x_j), \alpha^k_2(x_j))} \right].
\end{aligned}
\end{equation}

Moving back to our neural network architecture, the negative log-likelihood $-\ell$ serves as the loss function. In short, our aim is to learn $\bm w(x), \bm\alpha^1(x), \ldots, \bm\alpha^K(x)$ as functions of $x$ by minimizing \eqref{eq:full_like} using the powerful machinery of deep learning.

% To continue the calculation, we make use of a basic property of Beta function:
% \[
% \begin{aligned}
% &\int_{\Delta} \left( \prod_{i=1}^d p_i^{\sum_{l=1}^{m} \bm{1}(y^{(l)}= i)} \right) \sum_{k=1}^K w^k \frac1{\B(\bm\alpha^k)} \prod_{i=1}^d p_i^{\alpha^k_i -1}  \dx \bm p\\
% & = \sum_{k=1}^K w^k \frac{B\left (\alpha^k_1 + \sum_{l=1}^{m} \bm{1}(y^{(l)}= 1), \ldots, \alpha^k_d + \sum_{l=1}^{m} \bm{1}(y^{(l)}= d)\right)}{\B(\bm\alpha^k)}.
% \end{aligned}
% \]
%%Let $x_1, \ldots, x_n$ be the features of $n$ observational units, each of which are associated with labels $y_j^{(1)}, \ldots, y_j^{(m_j)}$ taking values of $1, 2$. Denote by $p(x)$ the probability of the label being 1 given $x$. A central piece of our model is to assume that $p(x)$ follows a Beta mixture distribution whose probability density is
%\[
%%f(p; x) = \sum_{k=1}^K w^k \frac{p^{\alpha^k_1 -1} (1-p)^{\alpha^k_2 -1}}{B(\alpha^k_1, \alpha^k_1)}
%%\]



\subsection{Credible Intervals}
\label{sec:credible-interval}

In this section, we discuss how to explicitly quantify the uncertainty for a freshly collected unit, say $x$. Let $\hat{\bm w}(x), \hat{\bm\alpha}^1(x), \ldots, \hat{\bm\alpha}^K(x)$ be the functions learned by the deep mixture networks. For the unit $x$, the estimated distribution of the probability $p(x)$ takes the form
\[
\hat f(p; x) = \sum_{k=1}^K \hat w^k(x) \frac{p^{\hat\alpha^k_1(x) -1} (1-p)^{\hat\alpha^k_2(x) -1}}{\B(\hat\alpha^k_1(x), \hat\alpha^k_2(x))}.
\]
Intuitively, if the density function $\hat f(p; x)$ is widely spread in the unit interval $[0, 1]$, much uncertainty is contained in the classification problem and, as a consequence, it is crucial to account for the uncertainty in interpreting the predictions of the neural networks.

To be concrete, in addition to giving a point estimator of the random probability $p_x$, $\hat f(p; x)$ can be used to construct one-sided and two-sided credible intervals for $p_x$. Intuitively, the expectation of this estimated density $\int_0^1 \hat f(p; x)\dx p$ is an unbiased estimator of $p_x$. Next, to construct credible intervals, let $\alpha \in (0, 1)$ be the nominal level. For a two-sided interval, let $\widehat Q_{\frac{\alpha}{2}}$ and $\widehat Q_{1 - \frac{\alpha}{2}}$ be the $\alpha/2$ and $1 - \alpha/2$ quantiles of the estimated density $\hat f$, respectively. Using the quantiles, the two-sided credible interval for $p_x$ at level $1 - \alpha$ takes the form
\[
\left[ \widehat Q_{\frac{\alpha}{2}}, \widehat Q_{1 - \frac{\alpha}{2}} \right].
\]
Likewise, the upper and lower credible intervals both at level $1 - \alpha$ are given as
\[
\left[0,  \widehat Q_{1 - \alpha}\right], \text{ and } \left[\widehat Q_{\alpha}, 1\right],
\]
respectively.

\subsection{Theoretical Analysis}\label{sec:universaility}

The uncertainty assessment carried out in Sections~\ref{sec:likelihood} and \ref{sec:credible-interval} considers the case where the density function is a Beta mixture. In this section, we show that this relaxation is mild in the sense that any density functions under certain regularity conditions can be approximated well by Beta mixtures. Explicitly, denote by $\mathcal P$ the set of all probability density functions $f$ on $[0, 1]$ with at most countable discontinuities that satisfy
\begin{align}\nonumber
\int_0^1 f(p) \left|\log f(p)\right| \dx p < \infty.
\end{align}
In \cite{article}, it is shown that any $f \in \mathcal{P}$ can be approximated arbitrarily close by a sequence of Beta mixtures. Precisely, we have the following theorem.
\begin{theorem}[\cite{article}]\label{thm1}
For any $f \in \mathcal{P}$ and any $\epsilon > 0$, there exists a Beta mixture distribution $f_{\B}$ such that
\begin{align}\nonumber
\mathrm{D}_{\mathrm{KL}} \left(f \| f_{\B} \right) \leq \epsilon,
\end{align}
where $\mathrm{D}_{\mathrm{KL}} (\cdot \| \cdot)$ denotes the Kullback-Leibler divergence.
\end{theorem}

This theorem shows the validity of approximating general distribution functions using Beta mixtures. In particular, Pinsker's inequality implies that the density can be approximated arbitrarily close in the total variance distance. In short, the proof of this result starts by recognizing that $f$ can be accurately approximated by piecewise constant functions on $[0,1]$ due to a countable number of discontinuities. Next, as shown in \cite{verdinelli1998bayesian,petrone2002consistency}, each constant piece is a limit of a sequence of Bernstein polynomials, which are infinite Beta mixtures with integer parameters.

For completeness, we remark it is unclear how to approximate $f(p; x)$ uniformly over $x$ using a sequence of Beta mixtures whose parameters are functions of $x$. It is likely that the approximation remains if the function $f(p, x)$ is smooth in $x$ in a certain sense, for example, $\int^1_0 |f(p; x) - f(p; x')| \dx p \le c \|x - x'\|$ for some $c > 0$. Provided that this is true,  the universal approximation theorem ensures that the functional $f$ can be arbitrarily approximated by Beta mixtures with parameters taking form of feed-forward networks. We leave this challenging problem for future investigation.


% \begin{align*}
% \sum_{(\alpha_k, \beta_k) \in \mathbb{N}^2_+} p_k \mathscr{B}(\alpha_k, \beta_k)
% \end{align*}
% %%We can see these pieces as intervals on $[0,1]$ as there are at most countable of $f$ on $[0,1]$. We can further use Beta mixture distribution to estimate $\widehat{f}$ on each of these intervals with Kullback-Leibler divergence as the measure. 
% There are substaintial literature state and interpret the validation of Beta mixture approximation. One approach to the interpretation and estimation mixtures with nonparametric methods \cite{verdinelli1998bayesian,petrone2002consistency} approximates bounded continuous density functions defined on $[0, 1]$ by \emph{Bernstein polynomials}. Bernstein polynomials is the infinite Beta mixtures with integer parameters.
% \begin{align*}
% \sum_{(\alpha_k, \beta_k) \in \mathbb{N}^2_+} p_k \mathscr{B}(\alpha_k, \beta_k)
% \end{align*}

% Obviously, a general case of Beta mixture distribution $f_{\omega}$ can at least approximate bounded continuous density functions on $[0, 1]$. 

% A brief idea of the proof is shown as follows. Given the property of $f \in \Omega$ stated above, we can approximate
% \begin{align*}
% \int_0^1 f(x) \left|\log f(x)\right| \mathrm{d}x
% \end{align*}
% by 
% \begin{align*}
% \int_0^1 \widehat{f}(x) \left|\log \widehat{f}(x)\right| \mathrm{d}x
% \end{align*}
% where $\widehat{f}$ is piecewise constant function on $[0,1]$. We can see these pieces as intervals on $[0,1]$ as there are at most countable of $f$ on $[0,1]$. We can further use Beta mixture distribution to estimate $\widehat{f}$ on each of these intervals with Kullback-Leibler divergence as the measure. 
% %%More details of proof are discussed in Appendix \ref{proof}.

%% Above, $w^k = w^k(x)$ and $\bm\alpha^k = \bm\alpha^k(x)$. 

\subsection{Extension to Multiple Classes}
\label{sec:extens-mult-labels}
To conclude, we extend our method to the general case of multi-class labels. The new setting follows seamlessly from the prior development except that now the labels $y_j^{(1)}, \ldots, y_j^{(m_j)}$ take values from $\{1, 2, \ldots, d \}$, where $d$ is the number of classes. Given a unit $x$, the multinomial distribution over $1, 2, \ldots, d$ is represented by $(p_1, \ldots, p_d)$, which, as a point in the simplex $\Delta = \{(c_1, \ldots, c_d): c_i \ge 0, c_1 + \cdots + c_d = 1\}$, is assumed to follow a Dirichlet mixture
\[
f(\bm p; x) = \sum_{k=1}^K w^k \frac1{\B(\bm\alpha^k)} \prod_{i=1}^d p_i^{\alpha^k_i -1}.
\]
Above, the generalized Beta function takes the form
\[
\B(\bm\alpha) = \frac{\prod_{i=1}^d \Gamma(\alpha_i)}{\Gamma(\alpha_1 + \cdots + \alpha_d)}.
\]
The likelihood of the observations $y_j^{(1)}, \ldots, y_j^{(m_j)}$ is
\[
L_j = \int_{\Delta} \left( \prod_{i=1}^d p_i^{S_{ij}} \right) \sum_{k=1}^K w^k(x_j) \frac1{\B (\bm\alpha^k(x_j))} \prod_{i=1}^d p_i^{\alpha^k_i(x_j) -1}  \dx \bm p.
\]
Recall that $S_{ij} = \sum_{l=1}^{m_j} \bm{1}(y_j^{(l)}= i)$. As such, the (full) negative log-likelihood is
\[
\footnotesize
\begin{aligned}
&-\ell(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K;  x_1, \bm y_1, \ldots, x_n, \bm y_n) \\
&= -\sum_{j=1}^n \log \left[\sum_{k=1}^K \frac{w^k(x_j)\B(\alpha^k_1(x_j)  + S_{1j}, \ldots, \alpha^k_d(x_j) + S_{dj})}{\B(\bm\alpha^k(x_j))} \right].
\end{aligned}
\normalsize
\]
This is the loss function to be minimized in the Dirichlet mixture networks.

% \[
% \begin{aligned}
% &-\ell(\bm w, \bm\alpha^1, \ldots, \bm\alpha^K;  x_1, \bm y_1, \ldots, x_n, \bm y_n) \\
% &= -\sum_{j=1}^n \log \left[ \int_{\Delta} \left( \prod_{i=1}^d p_i^{\sum_{l=1}^{m_j} \bm{1}(y_j^{(l)}= i)} \right) \sum_{k=1}^K w^k(x_j) \frac1{\B(\bm\alpha^k(x_j))} \prod_{i=1}^d p_i^{\alpha^k_i(x_j) -1}  \dx \bm p \right].
% \end{aligned}
% \]



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nipstemp"
%%% End:

